Interleaved Scene Graphs for Interleaved Text-and-Image Generation Assessment

Many real-world user queries (e.g. "How do to make egg fried rice?") could benefit from systems capable of generating responses with both textual steps with accompanying images, similar to a cookbook. Models designed to generate interleaved text and images face challenges in ensuring consistency within and across these modalities. To address these challenges, we present ISG, a comprehensive evaluation framework for interleaved text-and-image generation. ISG leverages a scene graph structure to capture relationships between text and image blocks, evaluating responses on four levels of granularity: holistic, structural, block-level, and image-specific. This multi-tiered evaluation allows for a nuanced assessment of consistency, coherence, and accuracy, and provides interpretable question-answer feedback. In conjunction with ISG, we introduce a benchmark, ISG-Bench, encompassing 1,150 samples across 8 categories and 21 subcategories. This benchmark dataset includes complex language-vision dependencies and golden answers to evaluate models effectively on vision-centric tasks such as style transfer, a challenging area for current models. Using ISG-Bench, we demonstrate that recent unified vision-language models perform poorly on generating interleaved content. While compositional approaches that combine separate language and image models show a 111% improvement over unified models at the holistic level, their performance remains suboptimal at both block and image levels. To facilitate future work, we develop ISG-Agent, a baseline agent employing a "plan-execute-refine" pipeline to invoke tools, achieving a 122% performance improvement.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> old/abstract_v1.tex <==
% The emergence of unified Transformer-based models has enabled simultaneous multimodal understanding and generation, showing promise in unifying both vision and language tasks with interleaved text-and-image generation. 
Unified Transformer-based models have enabled simultaneous multimodal understanding and generation, showing promise in unifying both vision and language tasks with interleaved text-and-image generation. 
However, assessing the performance of multimodal interleaved generation remains unexplored and challenging due to the complexity of interleaved content. 
In this paper, we design an automatic multi-granular evaluation framework \fullname (ISG) with four levels to evaluate accurate interleaved generation tasks, which converts multimodal queries into atomic questions, then perform visual question answering for precise verification.
Moreover, we propose \name, the first multimodal interleaved benchmark with concrete generation requirement consisting of 1,150 samples across 21 text-image generation tasks.
Additionally, we pioneer in a compositional agent framework \methodname to explore the upper bound of interleaved generation with agent workflow. 
In our experiments, 
we conduct a multi-granular evaluation of \evalname, demonstrating its potential for automatically evaluating interleaved generation consistent with ground truth and human preferences. 
Furthermore, comprehensive assessments of 10 interleaved generative frameworks reveal that unified models still lack basic accurate instruction-following capabilities, falling short even in structural requirements. 
Additionally, our \methodname outperforms other compositional frameworks in interleaved generation at various levels but still struggles with vision-dominated tasks. 
Our work offers valuable insights for advancing future research in interleaved text-and-image generation.
% instruction following and precise generation.


==> old/abstract_v2.tex <==
% The emergence of unified Transformer-based models has enabled simultaneous multimodal understanding and generation, showing promise in unifying both vision and language tasks with interleaved text-and-image generation. 
Unified Transformer-based models have enabled simultaneous multimodal understanding and generation, showing promise in unifying both vision and language tasks with interleaved text-and-image generation. 
However, assessing the performance of multimodal interleaved generation remains unexplored and challenging due to the complexity of interleaved content. 
We design an automatic multi-granular evaluation framework called \fullname (ISG). 
ISG evaluates generations across four levels of granularity; for each granular evaluation, ISG converts each query into a set of atomic questions, which probes for various aspects of correctness.
Using ISG, we introduce \name, the first multimodal interleaved benchmark with concrete generation requirements for 1,150 queries, spanning a diverse set of 21 text-image generation tasks.



In our experiments, we conduct a multi-granular evaluation of \evalname, demonstrating its potential for automatically evaluating interleaved generation consistent with ground truth and human preferences. 
Furthermore, comprehensive assessments of 10 interleaved generative frameworks reveal that unified models still lack basic accurate instruction-following capabilities, falling short even in structural requirements. 
Additionally, we introduce a baseline in a compositional agent framework \methodname to explore the upper bound of interleaved generation with agent workflow, outperforming other compositional frameworks in interleaved generation at various levels but still struggles with vision-dominated tasks. 
Our work offers valuable insights for advancing future research in interleaved generation.
% instruction following and precise generation.

==> old/intro_v1.tex <==


\section{Introduction}

% With the rapid development of generative models \citep{openai_gpt4o_2024, geminiteam2023gemini, baldridge2024imagen, xiao2024omnigenunifiedimagegeneration}, significant progress has been made in text generation tasks, such as creative writing \citep{yuan2022wordcraft, gomez2023confederacy}, open-ended chatting \citep{zheng2023judging, zhao2024wildchat}, and code generation \citep{chen2021evaluating,zhuo2024bigcodebench}, as well as image generation tasks including text-to-image \citep{rombach2022high, betker2023improving}, editing \citep{brooks2023instructpix2pix,fu2023guiding}, and sequential prediction \citep{zhang2024extdm,liu2024intelligent}. Recently, some transformer-based models such as Transfusion \citep{zhou2024transfusion}, Anole \citep{chern2024anole}, and VILA-U \citep{wu2024vila} have shown the unified vision-language understanding \citep{yue2024mmmu, yu2024mm} and generation capability \citep{huang2023t2i, koh2024generating}, making interleaved text-image generation possible and further advancing towards Artificial General Intelligence (AGI).

% Large Language Models have achieved significant progress in content generation across multiple modalities: 1) text generation such as creative writing, dialog, and code generation, and 2) image generation such as text-to-image, image editing and sequential prediction.
% Recently, several Transformer-based models, such as Transfusion \citep{zhou2024transfusion}, Anole \citep{chern2024anole}, and VILA-U \citep{wu2024vila}, have been proposed to unify  both the  understanding \citep{yue2024mmmu, yu2024mm} and generation capability \citep{huang2023t2i, koh2024generating} of both vision and language, making interleaved text-image generation possible and further advancing towards Artificial General Intelligence (AGI).
%Multimodal Large Language Models (MLLMs) have made significant advancements in content generation across multiple modalities, including: 1) text generation, such as creative writing~\citep{yuan2022wordcraft, gomez2023confederacy}, dialogue~\citep{zheng2023judging, zhao2024wildchat}, and code generation~\citep{chen2021evaluating,zhuo2024bigcodebench}, and 2) image generation, encompassing text-to-image synthesis~\citep{rombach2022high, betker2023improving}, and image editing~\citep{brooks2023instructpix2pix,fu2023guiding}. Recently, several Transformer-based models—such as Transfusion~\citep{zhou2024transfusion}, Anole~\citep{chern2024anole}, and VILA-U~\citep{wu2024vila}—have been introduced to unify both  understanding~\citep{yue2024mmmu, yu2024mm} and generative capabilities~\citep{huang2023t2i, koh2024generating} of vision and language, enabling interleaved text-and-image generation.
% and pushing the boundaries towards Artificial General Intelligence (AGI).


% Imagine a scenario where a user faces a real-world vision-language problem such as \textit{``How to make egg fried rice?''} As shown in Figure \ref{fig:intro}, while MLLM chatbots generate only text and image generators produce visuals without text guidance, neither fully meets users' comprehensive needs. However, with the capability to generate text and images together, unified generative assistants can produce intuitive images that further illustrate the text content; while also expressing their thought processes through text output for vision-guided tasks, significantly improving their helpfulness.
% Figure~\ref{fig:intro} shows a real-world example to illustrate the interleaved text-image generation. Given a user query \textit{``How to make egg fried rice?''}, we can see that existing Multimodal Large Language Models (MLLMs) (e.g., LLaVA) only generate the corresponding receipt in textual format. While the image generative models (e.g., SD) only simply generate the visual receipt without textual guidance.
% We argue that these two models can not provide good experience to end users. Therefore, a unified model with the capability of generating interleaved texts and images are in pressing demand, since the interleaved texts and images can impress users complementarily with better user experience.
%Figure~\ref{fig:intro} presents a real-world example to illustrate interleaved text-image generation. Given a user query such as \textit{``How to make egg fried rice?''}, current MLLMs, like LLaVA~\citep{liu2024visual}, generate only a textual recipe, while image generative models, such as Stable Diffusion (SD)~\citep{rombach2022high}, produce a visual receipt without textual guidance. We argue that neither model delivers an optimal user experience. Therefore, there is a pressing need for a unified model capable of generating interleaved text and images, as this combination can provide a more engaging and complementary user experience.
Generative AI has seen rapid development in recent years. People can use (Multimodal) Large Language Models (MLLMs) to generate text and code~\citep{yuan2022wordcraft, gomez2023confederacy,zhuo2024bigcodebench}, as well as diffusion-based generative models to produce high-quality images and videos~\citep{rombach2022high, betker2023improving, blattmann2023stable}. 
% However, visual content generation and text generation are often done separately.
However, the generation of visual content and text is typically handled separately.
In practical applications, many creative tasks require interleaving visual content and text during multimodal content creation, such as writing storybooks \citep{huang2016visual} or generating illustrated instructions based on user queries \citep{miech2019howto100m}. 
% Recently, there has been an increasing number of works proposed for interleaved text-and-image generation~\citep{zhou2024transfusion, li2024mini, chern2024anole, wu2024vila}. 
% Unlike generating individual modalities—such as purely text or purely visual content—interleaved multimodal generation requires the model to produce more complex output structures based on input instructions, while still maintaining consistency and coherence across modalities as with single-modality generation. The challenges, specifically, are threefold: 1) ensuring high-level consistency, which refers to coherence in the text; 2) maintaining low-level consistency, or pixel-level coherence in the visuals; and 3) ensuring cross-modality consistency between the high-level text and low-level visuals. Achieving all three is difficult because it requires a deep understanding of the semantic structure behind the generated content. 
As illustrated in Figure~\ref{fig:intro}, when given a user query \textit{“How to make egg fried rice?”}, we expect an interleaved text-and-image generative model to produce outputs with internal structural consistency, rather than loosely related outputs generated in a unimodal fashion.


\begin{figure}[t]
    \centering
    \vspace{-1em}
    \includegraphics[width=0.98\linewidth]{figure/intro.pdf}
    \vspace{-1em}
    \caption{Illustration of differences of each generative model. \textbf{Left:} Text Generation; \textbf{Middle:} Image Generation; \textbf{Right:} Interleaved Text-and-Image Generation.}
    \label{fig:intro}
    \vspace{-1.0em}
\end{figure}

% To generate interleaved multimodal outputs with internal structural consistency, we must first emphasize the importance of this aspect during the evaluation phase. However, current benchmarks~\citep{chen2024comm,an2023openleaf,liu2024holistic} do not account for this. Highlighting the need for multimodal outputs to satisfy the consistency within their relatively complex internal structures during evaluation can lead to more fine-grained and interpretable assessments. This, in turn, provides more instructive constraints for guiding the generative process.

Despite the increasing enhancement and attention given to interleaved generative models~\citep{zhou2024transfusion, li2024mini, chern2024anole, wu2024vila}, evaluating their capabilities through benchmarks \citep{chen2024comm,an2023openleaf,liu2024holistic} still presents challenges: 
%Recently, there has been a growing number of works proposed for interleaved text-and-image generation~\citep{li2024mini, chern2024anole, wu2024vila}. 
%However, assessing their capabilities through benchmarks \citep{chen2024comm,an2023openleaf,liu2024holistic} remains underexplored, with several limitations that need to be addressed.
% However, evaluating their capabilities through benchmarks \citep{chen2024comm,an2023openleaf,liu2024holistic} still poses challenges:
% \textbf{1)} Previous benchmarks primarily focused on text tasks, requiring only textual input (with image content described in the query) and textual responses, which not adequately benchmark their multimodal understanding and generation capablities. 
\textbf{1)} Previous benchmarks primarily focused on text-based tasks, requiring only textual input (with image content described in the query) and textual responses, which do not adequately assess their multimodal understanding and generation capabilities.
% \textbf{2)} Their queries are open-ended free-form without reference answers, which can not assess their accurate instruction following and generation capabilities. 
% \textbf{2)} The queries in existing benchmarks are open-ended free-form without reference answers, resulting that they can not be utilized to assess their  instruction following and generation capabilities. 
\textbf{2)} The queries in existing benchmarks are open-ended and free-form without reference answers, making them unsuitable for evaluating instruction following and generation capabilities.
% \textbf{3)} Evaluation of interleaved generation is extremely hard, requiring more fine-grained and interpretable assessments of their generated images and text elements.
% \textbf{3)} Existing benchmarks are not sufficiently evaluated in fine-grained level and lack of interpretability, which are very significant for the interleaved text-and-image generation.
\textbf{3)} Existing benchmarks lack fine-grained and interpretable evaluation, which are crucial for assessing interleaved text-and-image generation.

% To mitigate these limitations, we first propose an automatic multi-granular evaluation framework \fullname (ISG), to assess the performance of interleaved generation across four levels (i.e., xxxx, xxxx, xxxx, and xxxx).
% Specifically, we curate queries by detailing the structural, block, and image levels, and leverage VQA \citep{hu2023tifa, lin2024evaluating} for automatic evaluation. 
% To validate the effectiveness of ISG, we further introduce a multimodal interleaved generative benchmark \name for multiple tasks, with 21 evaluation categories and 1,150 samples, all incorporating both language-vision dependencies and carefully collected golden answers. 

To this end, we propose an evaluation framework that interprets the input query into four levels: holistic, structural, block, and image, referred to as \fullname (ISG). Based on ISG, we generate a large number of reasoning questions about the internal structure of the interleaved multimodal generation output. These reasoning questions are then used for automatic evaluation via Visual Question Answering (VQA)~\citep{hu2023tifa}, allowing us to assess whether the internal structure of the interleaved multimodal generation is accurate during the evaluation phase.

Based on this framework, we introduce a multimodal interleaved generative benchmark, \name, covering multiple tasks with 21 evaluation categories and 1,150 samples, all of which require accurate interleaved text-and-image generation and integrate language-vision dependencies as well as carefully curated golden answers. 
In \name, we pioneer in introducing vision-centric interleaved generative tasks such as \textit{``Semantic Segmentation''}~\citep{li2022bridging}, to fill the blankness in previous benchmarks for a more comprehensive evaluation. Our extensive human evaluations at each stage of \evalname over \name demonstrate its effectiveness in assessing interleaved text-and-image generation.
% for a more comprehensive evaluation. Our extensive human evaluation for each step within \evalname and \name demonstrates its reliability in assessing accurate interleaved generation. 
% Additionally, we provided task-specific evaluation metrics to facilitate a comprehensive framework for multimodal interleaved generation assessment.

% To further explore the compositional framework of \name in evaluating interleaved text-and-image generation, we build a MLLM-based agent, \methodname, which generates interleaved text-image through a \textit{``Plan-Execute-Refine''} pipeline \citep{wang2024genartist}. 
% In particular, it xxxxxx, and subsequently xxxxxx.
% Experimental results show that \methodname excels in instruction-following and  interleaved text-and-image generation by composing multimodal understanding capability and advanced tools of multimodal generation based on MLLMs. 
Inspired by previous compositional generative framework with the state-of-the-art results \citep{gupta2023visual,suris2023vipergpt, ma2024m}, we 
%propose an agent framework \methodname as a pioneering exploration in interleaved text-and-image generation.
%To further investigate the compositional framework of \name in evaluating interleaved text-and-image generation, we 
pioneer in developing an MLLM-based agent, \methodname, which generates interleaved text and images through a \textit{``Plan-Execute-Refine''} pipeline \citep{wang2024genartist}. Specifically, it first provides a plan of tool-usage and subsequently executes these advanced tools for interleaved generation, followed by a refinement process for better text-and-image alignment and error fixing. 
% Experimental results on \name demonstrate that \methodname excels in instruction-following and accurate interleaved text-and-image generation by leveraging the multimodal understanding capabilities and advanced tools of MLLMs.

% To further explore the compositional framework for interleaved generation, we innovatively propose the first agent framework, \methodname, which generates interleaved text-image through a \textit{``Plan-Execute-Refine''} pipeline \citep{wang2024genartist}. \methodname is designed to excel in instruction-following and accurate interleaved generation by composing MLLM's multimodal understanding capability and advanced tools of multimodal generation. 

% Based on \name and \evalname, we assess the accurate generation and instruction-following capability among 9 accessible multimodal interleaved generative frameworks, including four recently popular unified models, four complementary frameworks, and our \methodname. 
% Based on \name and \evalname, we assess the accurate generation and instruction-following capability among, 
% We benchmark ten accessible interleaved text-and-image generative frameworks, including five recently popular unified models (\textit{i.e.}, Show-o~\cite{xie2024show}, Anole~\cite{chern2024anole}), four complementary frameworks (\textit{i.e.}, Claude + SD3~\cite{esser2024scaling}), and our \methodname.
% Empirical results show that current unified models still have significant room for improvement in both generation accuracy and quality.
% Furthermore, \methodname significantly outperforms other baselines, showcasing its superior accuracy and coherency in interleaved text-and-image generation, thus serving a strong baseline for further research.
% Additionally, we also observe that the vision-dominated tasks (\textit{e.g.}, \textit{``Style Transfer''}) present considerable challenges to models' instruction-following capabilities and generation accuracy, with all models and frameworks failing to maintain original fidelity in generated images.
We benchmark ten accessible interleaved text-and-image generative frameworks, including five recently popular unified models (e.g., Show-o~\citep{xie2024show}, Anole~\citep{chern2024anole}), four complementary frameworks (e.g., Claude + SD3~\citep{esser2024scaling}), and our proposed \methodname. Empirical results demonstrate that current unified models still exhibit significant room for improvement in both generation accuracy and quality. Notably, \methodname outperforms all other baselines, demonstrating superior accuracy and coherence in interleaved text-and-image generation, establishing it as a strong baseline for future research. Additionally, we observe that vision-dominated tasks (e.g., \textit{``Style Transfer''}) pose considerable challenges to models' instruction-following abilities and generation accuracy, with none of the models maintaining the original fidelity in generated images.
% \textcolor{red}{FIX THE REFERENCE ERRORs}
% We conclude by discussing several future directions for developing unified models and compositional frameworks, thereby providing valuable insights for future research in this field. 

% as well as addressing trustworthiness issues in interleaved generation, 


% Empirical results reveal that current unified models still have significant room for improvement in both generation accuracy and quality. \methodname outperforms all compositional frameworks, demonstrating superior accurate generation and text-image coherence, thus establishing a baseline for interleaved generative tasks. Vision-dominated tasks present considerable challenges to models' instruction-following capabilities and generation accuracy, with all models maintaining original fidelity in the generated images. We conclude by discussing future directions for developing unified models and compositional frameworks, as well as addressing trustworthiness concerns in multimodal interleaved generation, thereby providing valuable insights for future research in this field.

In summary, the contributions of this paper are four-fold:
\begin{itemize}[itemsep=0pt, leftmargin=*]
\item\textbf{An Automatic Evaluation Framework.} 
% We propose an automatic multi-level framework \evalname that evaluates interleaved generation in four levels—overall, structural, block, and image—for a comprehensive assessment.
We propose an automatic evaluation framework, \evalname, that assesses interleaved text-and-image generation across four levels—holistic, structural, block, and image—for a comprehensive assessment.

% \item\textbf{A Multimodal Interleaved Generative Benchmark.} 
\item\textbf{A New Benchmark.} 
% We construct the first multimodal interleaved generative benchmark \name, with 8 categories and 1,150 samples, all incorporating both language-vision dependencies and golden answers. 
% We construct the first benchmark \name for evaluating interleaved text-and-image generation tasks, covering 21 categories and 1,150 samples, all incorporating both language-vision dependencies and golden answers. 
We introduce \name, the first benchmark for accurate interleaved generation tasks, encompassing 21 categories and 1,150 samples, each integrating language-vision dependencies with corresponding golden answers.

\item\textbf{An Interleaved Generative Agent.} We introduce \methodname, a unified agent with integrated tool execution, designed to explore the upper bounds of interleaved generation tasks.

\item\textbf{Extensive Evaluation and Implications.} 
% We conduct extensive experiments to evaluate all current multimodal interleaved generation models and frameworks, as well as our proposed agent \methodname to explore task performance limits, offering valuable insights for future development.
% We conduct extensive experiments to evaluate all current multimodal interleaved generation models and frameworks, as well as our proposed \methodname, offering valuable implications for future study.
We conduct extensive experiments to evaluate current interleaved text-and-image generation models and frameworks, including our proposed \methodname, providing valuable insights for future research.
\end{itemize}


==> old/intro_v2.tex <==


\section{Introduction}

% PARAGRAPH 1: Set up the problem and motivate it.
With the proliferation of multimodal language models, it has become apparent that users want models that can simultaneously generate both text as well as images~\citep{huang2016visual,miech2019howto100m}. Consider a scenario where a user asks \textit{``How to make egg fried rice?''} (Figure~\ref{fig:intro}). Of course, answer this query in language—with a list of steps—is one reasonable answer; a more ecological response could follow the style of cookbooks: by creating intermediate images of the cooking process alongside those steps. Enabling such responses is possible by leveraging a language generation model~\citep{yuan2022wordcraft, gomez2023confederacy,zhuo2024bigcodebench} in tandem with a separate image generation model~\citep{rombach2022high, betker2023improving, blattmann2023stable}. But the need for dual models slows down inference as both models have to be loaded and run in sequence. 
Many practical applications, such as writing storybooks~\citep{huang2016visual} or generating illustrated instructions~\citep{miech2019howto100m}, require generating interleaved images and text. 


% PARAGRAPH 2: Set up the need for benchmarks and cite what is lacking in existing benchmarks.
The community has begun designing unified models with the capability of generating interleaved texts and images for such use cases~\citep{zhou2024transfusion, li2024mini, chern2024anole, wu2024vila}. 
Generating multiple modalities is challenging. The generations between modalities need to maintain consistency, between multiple images, between multiple sentences, and across the generated images and sentences.
Benchmarks for such challenges are still in its infancy~\citep{chen2024comm}.
\textbf{1)} Previous benchmarks primarily focus on text outputs, which do not adequately assess their multimodal understanding and generation capabilities~\citep{liu2024holistic}.
\textbf{2)} The queries in existing benchmarks are open-ended and free-form without reference answers, making them ambiguous for evaluating instruction following and generation capabilities~\citep{an2023openleaf}.
\textbf{3)} Existing benchmarks lack fine-grained and interpretable evaluation, which are crucial for assessing when and why models fail~\citep{xia2024mmie}.


\begin{figure}[t]
    \centering
    % \vspace{-1em}
    \includegraphics[width=0.98\linewidth]{figure/intro.pdf}
    % \vspace{-1em}
    \caption{Illustration of differences of each generative model. \textbf{Left:} Text Generation; \textbf{Middle:} Image Generation; \textbf{Right:} Interleaved Text-and-Image Generation.}
    \label{fig:intro}
    \vspace{-1.0em}
\end{figure}


% PARAGRAPH 3: What is the high-level contribution and insight?
In this paper, we propose an evaluation framework for interleaved image-and-text generation, \fullname (ISG), into four levels for assessment: holistic, structural, block, and image. \evalname can automatically translate the user's query into requirements in each level for fine-grained evaluation and provide more interpretable assessments, filling the blankness in previous research. These requirements are then transformed into questions for automatic evaluation via Visual Question Answering (VQA)~\citep{hu2023tifa}, allowing us to assess whether the internal structure and atomic content (\textit{i.e.}, image or text block within the whole answer) of the interleaved multimodal generation strictly follow user's instructions. Our evaluations of \evalname with human-annotated judgments demonstrate its efficacy and alignment with humans in all four levels, outperforming previous MLLM-as-a-Judge \citep{chen2024mllm} in alignment with humans and convincing its potential in assessing interleaved generation.


% PARAGRAPH 4: Introduce the benchmark.
Based on \evalname, we collect a large number of queries from various domains that inertial requires interleaved multimodal generation output to answer, all with detailed instructions for \evalname to evaluate these answers. \name consists of 8 categories, 21 subcategories, and 1,150 samples, all incorporating both language-vision dependencies and golden answers to solve the above-mentioned problems. All samples are meticulously collected from previous datasets or built from scratch for high quality. Moreover, we pioneer in proposing vision-dominate tasks such as \textit{``Style Transfer''} to evaluate those unified models comprehensively and requirements for accurate image generation in specific tasks. Table \ref{tab:compare_benchmark} shows the difference between current interleaved benchmarks and datasets, building a solid platform for interleaved generation assessments. 

% PARAGRAPH 5: Talk about the existing models and their evaluations. How well do they work? Why and when do they fail? 
We benchmark nine accessible interleaved text-and-image generative frameworks, including five recently popular unified models (\textit{e.g.}, Show-o~\citep{xie2024show}, Anole~\citep{chern2024anole}), four compositional frameworks (\textit{e.g.}, Claude + SD3~\citep{esser2024scaling}). Empirical results demonstrate that current unified models still exhibit significant room for improvement in both instruction following and generation quality. Compositional frameworks, on the other hand, outperform unified models in language-guided tasks (\textit{e.g.}, \textit{``VQA''}) with high-quality image-and-text content especially at holistic levels, while still falling short in block and image levels for accurate generation due to their separate structure for understanding and generation. Additionally, we observe that vision-dominated tasks (\textit{e.g.}, \textit{``Style Transfer''}) pose considerable challenges to models' generation accuracy and quality, with none of the models maintaining the original fidelity in generated images when compared to human-annotated golden answer.


% PARAGRAPH 6: Finally mention the agent and how it was built and what the main takeaways are.
Finally, we pioneer in developing an MLLM-based agent \methodname inspired by previous compositional framework with the state-of-the-art results \citep{gupta2023visual,suris2023vipergpt, ma2024m}, which generates interleaved text and images through a \textit{``Plan-Execute-Refine''} pipeline \citep{wang2024genartist}. Specifically, it first provides a plan of tool usage and subsequently executes these advanced tools for interleaved generation, followed by a refinement process for better text-and-image alignment and error fixing. Notably, \methodname outperforms all other baselines, demonstrating superior accuracy and coherence in interleaved text-and-image generation, establishing it as a strong baseline for future research. 

% Based on ISG, we introduce a multimodal interleaved generative benchmark, \name, covering multiple tasks with 21 evaluation categories and 1,150 samples, all of which require accurate interleaved text-and-image generation and integrate language-vision dependencies as well as carefully curated golden answers. 
% Our extensive human evaluations at each stage of \evalname over \name demonstrate its effectiveness in assessing interleaved text-and-image generation.
% for a more comprehensive evaluation. Our extensive human evaluation for each step within \evalname and \name demonstrates its reliability in assessing accurate interleaved generation. 
% Additionally, we provided task-specific evaluation metrics to facilitate a comprehensive framework for multimodal interleaved generation assessment.

% To further explore the compositional framework of \name in evaluating interleaved text-and-image generation, we build a MLLM-based agent, \methodname, which generates interleaved text-image through a \textit{``Plan-Execute-Refine''} pipeline \citep{wang2024genartist}. 
% In particular, it xxxxxx, and subsequently xxxxxx.
% Experimental results show that \methodname excels in instruction-following and  interleaved text-and-image generation by composing multimodal understanding capability and advanced tools of multimodal generation based on MLLMs. 

%propose an agent framework \methodname as a pioneering exploration in interleaved text-and-image generation.
%To further investigate the compositional framework of \name in evaluating interleaved text-and-image generation, we 

% Experimental results on \name demonstrate that \methodname excels in instruction-following and accurate interleaved text-and-image generation by leveraging the multimodal understanding capabilities and advanced tools of MLLMs.

% To further explore the compositional framework for interleaved generation, we innovatively propose the first agent framework, \methodname, which generates interleaved text-image through a \textit{``Plan-Execute-Refine''} pipeline \citep{wang2024genartist}. \methodname is designed to excel in instruction-following and accurate interleaved generation by composing MLLM's multimodal understanding capability and advanced tools of multimodal generation. 

% Based on \name and \evalname, we assess the accurate generation and instruction-following capability among 9 accessible multimodal interleaved generative frameworks, including four recently popular unified models, four complementary frameworks, and our \methodname. 
% Based on \name and \evalname, we assess the accurate generation and instruction-following capability among, 
% We benchmark ten accessible interleaved text-and-image generative frameworks, including five recently popular unified models (\textit{i.e.}, Show-o~\cite{xie2024show}, Anole~\cite{chern2024anole}), four complementary frameworks (\textit{i.e.}, Claude + SD3~\cite{esser2024scaling}), and our \methodname.
% Empirical results show that current unified models still have significant room for improvement in both generation accuracy and quality.
% Furthermore, \methodname significantly outperforms other baselines, showcasing its superior accuracy and coherency in interleaved text-and-image generation, thus serving a strong baseline for further research.
% Additionally, we also observe that the vision-dominated tasks (\textit{e.g.}, \textit{``Style Transfer''}) present considerable challenges to models' instruction-following capabilities and generation accuracy, with all models and frameworks failing to maintain original fidelity in generated images.
% \textcolor{red}{FIX THE REFERENCE ERRORs}
% We conclude by discussing several future directions for developing unified models and compositional frameworks, thereby providing valuable insights for future research in this field. 

% as well as addressing trustworthiness issues in interleaved generation, 


% Empirical results reveal that current unified models still have significant room for improvement in both generation accuracy and quality. \methodname outperforms all compositional frameworks, demonstrating superior accurate generation and text-image coherence, thus establishing a baseline for interleaved generative tasks. Vision-dominated tasks present considerable challenges to models' instruction-following capabilities and generation accuracy, with all models maintaining original fidelity in the generated images. We conclude by discussing future directions for developing unified models and compositional frameworks, as well as addressing trustworthiness concerns in multimodal interleaved generation, thereby providing valuable insights for future research in this field.

% In summary, the contributions of this paper are four-fold:
% \begin{itemize}[itemsep=0pt, leftmargin=*]
% \item\textbf{An Automatic Evaluation Framework.} 
% We propose an automatic multi-level framework \evalname that evaluates interleaved generation in four levels—overall, structural, block, and image—for a comprehensive assessment.
% We propose an automatic evaluation framework, \evalname, that assesses interleaved text-and-image generation across four levels—holistic, structural, block, and image—for a comprehensive assessment.

% \item\textbf{A Multimodal Interleaved Generative Benchmark.} 
% \item\textbf{A New Benchmark.} 
% We construct the first multimodal interleaved generative benchmark \name, with 8 categories and 1,150 samples, all incorporating both language-vision dependencies and golden answers. 
% We construct the first benchmark \name for evaluating interleaved text-and-image generation tasks, covering 21 categories and 1,150 samples, all incorporating both language-vision dependencies and golden answers. 
% We introduce \name, the first benchmark for accurate interleaved generation tasks, encompassing 21 categories and 1,150 samples, each integrating language-vision dependencies with corresponding golden answers.

% \item\textbf{An Interleaved Generative Agent.} We introduce \methodname, a unified agent with integrated tool execution, designed to explore the upper bounds of interleaved generation tasks.

% \item\textbf{Extensive Evaluation and Implications.} 
% We conduct extensive experiments to evaluate current interleaved text-and-image generation models and frameworks, including our proposed \methodname, providing valuable insights for future research.
% \end{itemize}


==> old/method_v1.tex <==
% \vspace{-0.5em}
\begin{figure}[t]
    \centering
    \vspace{-1em}
    \includegraphics[width=1\linewidth]{figure/evaluation.pdf}
    \vspace{-1.5em}
    \caption{An overview of \evalname. \ranjay{Look at my other papers. The figures need to be completely independent of the main text. Your captions need to convey all the important information. Some readers only read the abstract and the figure/table captions. They will not be able to make sense of this figure.}}
    \label{fig:ISG}
    \vspace{-1em}
\end{figure}

\section{Interleaved Scene Graph}
We introduce \evalname (Figure~\ref{fig:ISG}), a comprehensive automatic evaluation framework for interleaved text-and-image generation assessment.
Using \evalname, we introduce \name, a benchmark for evaluating image-and-text generation.

% the first accurate interleaved text-and-image generation benchmark in Sec.~\ref{benchmark}, \name (Figure~\ref{fig:pie}), accompanied by automatic, atomic, and multi-granular evaluation methods \evalname (Figure~\ref{fig:ISG}) designed to evaluate accurate interleaved generation in Sec.~\ref{evaluation}. Then, we propose an compositional agent framework \methodname (Figure~\ref{fig:agent}) that designed as an exploratory study for interleaved generation in Sec.~\ref{agent}.

% \subsection{\fullname}
\subsection{The evaluation framework}
\label{evaluation}
 The framework automatically interprets well-constructed queries into a scene-graph-like structure, where text and image blocks serve as nodes and their relationships as edges. Based on this graph representation, we can perform comprehensively four-level assessment: holistic, structural, block, and image. At the macro level, Structural and Holistic evaluations analyze the overall response coherence and quality; while Block and Image evaluations assess how accurately each content module adheres to the user's instructions. Together, these four evaluation levels enable systematic assessment of interleaved generation quality, detailed as follows:

% Let \( P = \{B_{1}, B_{2}, \ldots, B_{n}\} \) represent the input prompt, where \( B_i \in \{I, T\} \) denotes a block that can be either an image (\(I\)) or text (\(T\)). We then use an MLLM to analyze the multimodal input and predict the output structure, denoted as \( \operatorname{MLLM}(prompt_1, P) = \{B_{n+1}, B_{n+2}, \ldots, B_m\} \), which details a sequence of interleaved multimedia elements. 
\begin{itemize}[itemsep=0pt, leftmargin=*]
    \item \textbf{Structural.} We evaluate structural-level interleaved generation for whether its generation strictly follows the structure requirement in user's query. As shown in Figure \ref{fig:ISG}, given structural requirement \textit{``generate image first followed by an instruction''}, the correct structure should consist of 4 images interleaved by 4 text blocks. We leverage an LLM to predict the generated structure based on the query and subsequently evaluate answers through direct structural matching.
    \item \textbf{Holistic.} 
    We conduct the holistic-level evaluation for assessing the overall text-image alignment, coherence, and helpfulness by inputting the multimodal query, response, and human-annotated golden answer into an MLLM, which then outputs judgments on the entire answer. Building on previous settings~\citep{an2023openleaf, liu2024holistic}, we enhance the process by employing MLLM-as-a-Judge \citep{chen2024mllm} with golden answers and the \textit{``Analyze-then-Judge''} Chain-of-Thought (CoT)~\citep{wei2022chain}. This allows for a more human-aligned evaluation, assessing generation quality, text-image alignment, and helpfulness to yield a comprehensive score.
    \item \textbf{Block.} 
    We evaluate block-level for fine-grained and accurate relation-aware interleaved generation by interpreting the query into various atomic block-to-block questions and subsequently leveraging VQA for evaluation.
    We initially represent the prompt \(P\) as subject-object-relation tuples \((\text{sub}, \text{obj}, r)\), such as \textit{\(<\text{Text 1, Image 1, Describe}>\)} in the example of Figure \ref{fig:ISG}, where \(\{\text{sub}, \text{obj}\}\) are nodes that denotes image or text block and \(r\) is edge that denotes an atomic open-vocabulary requirement. Subsequently, we generate questions from these tuples and evaluate them using the VQA module, with MLLMs providing \textit{``Yes-or-No''} and \textit{``1-10 score''} answers. We also attempt to use CLIPScore~\citep{hessel2021clipscore} for assessing text-image relations, but it fails due to the text block exceeding the text encoder's limit of 77 tokens.
    \item \textbf{Image.} 
    % We evaluate image-level interleaved generation following $\textbf{Prompt + Image}\rightarrow \textbf{Questions}\rightarrow \textbf{Image-Level VQA}$, which transform multimodal queries into dependent-aware tuples comprising entities, relations, and attributes, each associated with specific generated images, especially for vision-dominate tasks like \textit{``Style Transfer''}. 
    We conduct image-level task-specific assessments for accurate image content generation. We transform multimodal queries into dependency-aware tuples that comprise entities, relations, and attributes, each linked to specific generated images, particularly for vision-dominant tasks such as \textit{``Style Transfer''} and \textit{``Multi-Angle Object''} that have concrete referential answers, whereas the \textit{``Painting''} task requires only the accurate generation of the final image. In contrast, tasks such as \textit{``HowTo''} demand the inclusion of specific objects but allow flexibility in other aspects. We categorize tasks based on the requirement of image generation in the answers as shown in Table \ref{tab: benchmark details}.
    These tuples might include \textit{$<$Image 1, Entity, Cat$>$} and \textit{$<$Image 1, Relation, Cat, on the right of, Dog$>$}. Subsequently, we employ an LLM to generate questions with dependencies and evaluate image generation using these questions via a VQA module~\citep{cho2023davidsonian}.
    % Creative tasks like \textit{``Visual Story Telling''} lack definite answers and thus have no strict generation requirements. To evaluate these accurate image generation requirements, we leverage multimodal DSG \citep{cho2023davidsonian} as mentioned above.
\end{itemize}

% Each level (except holistic) leveraging MLLM is implemented with few-shot examples for in-context learning \citep{dong2022survey} and carefully verified compared to human-annotated ground truth. Refer to Section~\ref{evaluating ISG} for evaluating \name and Appendix~\ref{Appendix: ISG details} for technical details.
Each level, except the holistic one, leverages MLLM implemented with few-shot examples for in-context learning~\citep{dong2022survey} and is carefully verified against human-annotated ground truth. For the evaluation of \name, refer to Section~\ref{evaluating ISG}, and for technical details, see Appendix~\ref{Appendix: ISG details}.

% \header{Additional Evaluation at Different Granularity.}
% We also conduct evaluations at various granularities using task-specific metrics for a more comprehensive study. At the global level, we follow previous study \citep{an2023openleaf, liu2024holistic} to employ MLLM-as-a-Judge to compare with human-collected golden answers, assessing generation quality and accuracy using different rubrics to yield a general score. For different modal, we employ specialized metrics.  At the image level, 

\begin{figure}[t]
    \centering
    \vspace{-1em}
    \includegraphics[width=0.85\linewidth]{figure/pie.pdf}
    \vspace{-0.5em}
    \caption{\textbf{Left:} An overview of hierarchical categories in \name; \textbf{Right:} Distributions of the length of textual content and images for queries and golden answers.}
    \label{fig:pie}
    % \vspace{-0.5em}
\end{figure}


\begin{table}[t]
    \centering
        \caption{Task definitions and additional evaluation dimensions for \name. \textbf{Modal:} dominant modality in response evaluation; \textbf{Image:} the level of accurate image generation requirements.}
    \label{tab: benchmark details}
    \vspace{-1em}
    \renewcommand\arraystretch{1.1}
     \begin{threeparttable}
\resizebox{\linewidth}{!}{
\begin{tabular}{llcclc}
\toprule[1.5pt]
\textbf{Task} &
  \textbf{Description} &
  \textbf{Modal} &
  \textbf{Image} &
  \textbf{Subtask} &
  \textbf{\# Sample}  \\ \midrule
  \multirow{4}{*}{Style Transfer} &
  \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Generate a sequence of transformed\\ images with corresponding text\\ descriptions.\end{tabular}} &
  \multirow{4}{*}{\faImage} &
  \multirow{4}{*}{\faBatteryFull} &
  Art Style Transfer &
  50 \\
 &
   &
   &
   &
  Scene Attribute Transfer &
  50 \\
 &
   &
   &
   &
  Photo Variation &
  50 \\
 &
   &
   &
   &
  Portrait Variation &
  50 \\ \midrule
\multirow{3}{*}{Image Decomposition} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Segment input image into visual\\ elements with text descriptions.\end{tabular}} &
  \multirow{3}{*}{\faImage} &
  \multirow{3}{*}{\faBatteryFull} &
  Realistic Image Object Decomposition &
  50 \\
 &
   &
   &
   &
  Synthetic Image Object Decomposition &
  50 \\
 &
   &
   &
   &
  Semantic Decomposition &
  50 \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}3D Scene \\ Transformation\end{tabular}} &
  \multirow{2}{*}{3D Transformation for images} &
  \multirow{2}{*}{\faImage} &
  \multirow{2}{*}{\faBatteryFull} &
  Multi-view Scene Generation &
  50 \\
 &
   &
   &
   &
  Multi-Angle Object Generation &
  50 \\ \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Progressive Image\\ Transformation\end{tabular}} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Generate a sequence of images\\ that show gradual changes\end{tabular}} &
  \multirow{3}{*}{\faImage} &
  \multirow{3}{*}{\faBatteryHalf} &
  Text-guided Animation &
  50 \\
 &
   &
   &
   &
  Image-guided Animation &
  50 \\
 &
   &
   &
   &
  Attribute-guided Image Generation &
  50 \\ \midrule
\multirow{2}{*}{Temporal Prediction} &
  \multirow{2}{*}{Forecast future or past sequences} &
  \multirow{2}{*}{\faImage\  \faFont} &
  \multirow{2}{*}{\faBatteryHalf} &
  Real-world Simulation &
  50 \\
 &
   &
   &
   &
  Painting Process Generation &
  50 \\ \midrule
  \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Image-Text \\ Complementation\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Generate complementary visual or\\ textual content\end{tabular}} &
  \multirow{2}{*}{\faImage\  \faFont} &
  \multirow{2}{*}{\faBatteryEmpty} &
  HowTo &
  100* \\
 &
   &
   &
   &
  Scientific Phenomenon Explanation &
  50 \\ \midrule
\multirow{3}{*}{Visual Story Telling} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Tell a coherent narrative story with\\ images and texts\end{tabular}} &
  \multirow{3}{*}{\faImage\  \faFont} &
  \multirow{3}{*}{\faBatteryEmpty} &
  Image-based Visual Storytelling &
  50 \\
 &
   &
   &
   &
  Text-based Visual Storytelling &
  50 \\
 &
   &
   &
   &
  Image \& Text-based Visual Storytelling &
  50 \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}VQA with Image\\ Generation\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Provide texts and relevant images\\ to answer the question\end{tabular}} &
  \multirow{2}{*}{\faFont} &
  \multirow{2}{*}{\faBatteryEmpty} &
  Object Q\&A and Explanation &
  100* \\
 &
   &
   &
   &
  Historical Event/Artifact Analysis &
  50 \\ \bottomrule[1.5pt]
\end{tabular}
}
    \begin{tablenotes}
        \scriptsize
        \item[] \faBatteryFull~ denotes accurate image generation requirement for all objects, \faBatteryHalf~ for main objects, and \faBatteryEmpty~ for no requirement.\\
        % \noindent \fullcirc ~ means using ground truth as the true answer, \halfcirc ~means using ground truth as the golden answer, \emptycirc~means no standard answer provided.\\
        \noindent * For some datasets, we constructed 100 samples because they are more common in life.
    \end{tablenotes}
      \end{threeparttable}
      \vspace{-1.5em}
\end{table}


\subsection{The Benchmark}
\label{benchmark}
% We introduce \name, the first multi-task interleaved text-and-image generative benchmark, to assess the multimodal understanding and \textbf{accurate} generating capabilities across various tasks. 
Based on \evalname, we develop the first benchmark, termed \name, for interleaved text-and-image generation to assess multimodal understanding and generation capabilities across various tasks.
% As shown in Table~\ref{tab: benchmark details}, \name is categorical-balanced, consisting of 1,150 samples, covering 21 subtasks across 8 daily interleaved generative scenarios. 
% All queries in samples are with detailed instruction and structural requirement like \textit{``Generate four images and provide a brief text description after your generated image.''} to assess both instructions following capability and accurate generation capability. 
% Every query is designed as \textbf{1)} vision-language dependent, which means the query cannot be addressed with the information in only a single modality and \textbf{2)} paired with a carefully collected golden reference answer. 
% All samples are collected and selected by authors with cross-validation and BertScore~\citep{zhang2019bertscore} for similarity filtering, detailed in Appendix~\ref{Appendix: Human Annotation}.
As shown in Table~\ref{tab: benchmark details}, \name consists of a categorically balanced dataset of 1,150 samples, covering 21 subtasks across 8 daily interleaved generative scenarios. 
Each sample includes detailed instructions and structural requirements, such as \textit{``Generate four images and provide a brief text description after your generated image,''} to evaluate both instruction-following capability and interleaved generation ability. Every query is designed to be \textbf{1)} vision-language dependent, meaning it cannot be addressed using information from a single modality alone, and \textbf{2)} paired with a carefully collected golden reference answer. All samples are collected and manually selected by the authors using cross-validation and BertScore~\citep{zhang2019bertscore} for similarity filtering, as detailed in Appendix~\ref{Appendix: Human Annotation}.

\header{Data Collection and Quality Control.} 
% Our benchmark collections mainly involve three stages. Firstly, we go through current existing datasets following the task definition and retrieval of high-quality and non-overlap vision metadata serving as the vision information in query and golden answer, with some collected by ourselves (\textit{e.g.}, \textit{``Multi-View Scene Generation''}). 
Our benchmark collections involve three main stages. First, we review existing datasets according to the task definition and retrieve high-quality, non-overlapping vision metadata to serve as the visual information in both the query and the golden answer, with some data collected by ourselves (\textit{e.g.}, \textit{``Multi-View Scene Generation''}). 
% Then, we curate natural language queries that refer to the images for automatic evaluation of these queries. 
% We also give the required structure of the output in the queries. MLLMs are leveraged to construct textual answers according to each task, with further examination by human annotators to ensure their accuracy. 
% Given the arising data contamination concerns of foundation models~\citep{balloccu2024leak, xu2024benchmark}, annotators are advised to construct free-form queries and build the whole query and golden answer from scratch. 
We then curate natural language queries that reference the images for automatic evaluation. Each query specifies the required structure of the output. MLLMs are employed to generate textual answers for each task, which are subsequently reviewed by human annotators to ensure accuracy. Due to concerns about data contamination in foundation models~\citep{balloccu2024leak, xu2024benchmark}, annotators are instructed to create free-form queries and develop both the query and the corresponding golden answer from scratch.
% Finally, we gain a diverse and high-quality interleaved multimodal benchmark with query-answer pairs from various sources. 
% To further control the quality of our samples, we perform cross-validation among different annotators for format and typo checking. The detailed definition, collection pipeline, and some extra examples are provided in Appendix~\ref{detailed benchmark construction}.
Finally, we obtain a diverse and high-quality interleaved multimodal benchmark with query-answer pairs sourced from various origins. To ensure the quality of our samples, we conduct cross-validation among different annotators for format consistency and typo checking. Detailed definitions, the collection pipeline, and additional examples are provided in Appendix~\ref{detailed benchmark construction}.

\header{Modality Specific Assessment.} We categorize each task within our \name into three modes (i.e., ) for their primary modality contributing to the output via decision tree \citep{}. For example, the \textit{``HowTo''} task requires both vision and language content to solve the problem, and \textit{``Art Style Transfer''} requires mainly on vision generation; while \textit{``VQA with Image Generation''} primarily relies on textual output, where the quality and accuracy of answers is mainly attributed to the language component, with generated images serving as complementary information.


% As shown in Table~\ref{tab: benchmark details}, in addition to categorizing tasks with definitions, we also provide two following dimensions for a more comprehensive understanding for each task:
% In addition to categorizing tasks with definitions, we also provide two additional dimensions for a more comprehensive understanding of each task, as shown in Table~\ref{tab: benchmark details}.
% \begin{itemize}[itemsep=0pt, leftmargin=*]
%     \item \textbf{Modality Domination.} 
    
    
%     \item \textbf{Accurate Image Generation.} 
%     % We further categorize tasks based on the requirement for image generation in answers. For instance, tasks such as \textit{``Multi-Angle Object''} tasks has concrete referential answers. In contrast, \textit{``Painting''} task only requires accurate generation for the final image and tasks like \textit{``HowTo''} require specific objects to appear but allow flexibility in other aspects. 
%     We further categorize tasks based on the requirement of image generation in the answers. For example, tasks like \textit{``Multi-Angle Object''} have concrete referential answers, whereas the \textit{``Painting''} task requires only the accurate generation of the final image. In contrast, tasks such as \textit{``HowTo''} demand the inclusion of specific objects but allow flexibility in other aspects.
%     % Creative tasks like \textit{``Visual Story Telling''} lack definite answers and thus have no strict generation requirements. To evaluate these accurate image generation requirements, we leverage multimodal DSG \citep{cho2023davidsonian} as mentioned above.
%     Creative tasks such as \textit{``Visual Storytelling''} lack definitive answers and therefore do not have strict generation requirements. To evaluate these image generation requirements accurately, we utilize multimodal DSG~\citep{cho2023davidsonian} as previously mentioned.
% \end{itemize}
